Privacy Preserving Stream Analytics: The Marriage of Randomized Response and Approximate Computing

How to preserve users' privacy while supporting high-utility analytics for low-latency stream processing? To answer this question: we describe the design, implementation, and evaluation of PRIVAPPROX, a data analytics system for privacy-preserving stream processing. PRIVAPPROX provides three properties: (i) Privacy: zero-knowledge privacy guarantees for users, a privacy bound tighter than the state-of-the-art differential privacy; (ii) Utility: an interface for data analysts to systematically explore the trade-offs between the output accuracy (with error-estimation) and query execution budget; (iii) Latency: near real-time stream processing based on a scalable "synchronization-free" distributed architecture. The key idea behind our approach is to marry two existing techniques together: namely, sampling (used in the context of approximate computing) and randomized response (used in the context of privacy-preserving analytics). The resulting marriage is complementary - it achieves stronger privacy guarantees and also improves performance, a necessary ingredient for achieving low-latency stream analytics.

==> benchmarks.tex <==
%\subsection{Micro-benchmarks}
%\label{subsec:microbenchmarks}
%
%\input{figuresTex/fig-benchmark-error}
%\input{figuresTex/fig-num-answers-error}
%\input{figuresTex/fig-fraction-yes-error}
%\input{figuresTex/fig-splitx-comparison}
%
%We first conducted micro-benchmarks to analyze the impact of the sampling and randomizing parameter selection on the utility and the user privacy (see $\S$~\ref{subsubsec:sampling-randomizing}), as well as the impact of the number of participated {\em Clients} and the fraction of origin truthful `yes' answers on the utility. Then, to measure the overhead of crypto operations of \projecttitle and previous systems, we built micro-benchmarks on a laptop, a smartphone and a high-performance server. Finally, we conducted an experiments with 2 cluster nodes to measure latency of components in our system with a previous system, that has a similar architecture with our system, namely {\em SplitX}~\cite{Chen-2013}. Each result of experiments is generated after 100 independent runs.
%%a MacBook Air laptop with a 2,2 GHz Intel Core i7 CPU, 8GB of RAM running OS X Yonsemite as well as on a smartphone with a 1 GHz CPU running Android 4.1.2.
%
%\subsubsection{ What is the effect of varying sampling and randomizing parameters $r$, $p$ and $q$?}
%\label{subsubsec:sampling-randomizing}
%We study the effect of sampling and randomizing parameters on the utility and user privacy by applying our sampling and randomizing mechanism to  synthetic datasets. For this experiment, we first randomly generate $10,000$ original answers with 80\% of them are 'yes`. Then, we measure the utility and the privacy with different values of the parameters by using the equation~\ref{thrm:zkp} and equation~\ref{eq:accuracyloss}, respectively.
%
%Figure \ref{fig:benchmark-error} depicts the utility with different values of the sampling and randomizing parameters, whereas Figure~\ref{fig:case-study-privacy} represents the privacy with various values of the sampling and randomizing parameters. The smaller accuracy loss $\eta$ means higher utility, and smaller privacy level $\epsilon$ means stronger privacy. The sampling and randomizing parameters handle the trade-off between the utility and the privacy guarantee of the query results. 
%
%To analyze the effect of the randomizing parameters $p$ and $q$ on the utility and the privacy guarantee, the sampling parameter is set to $60$\%. The results of this experiment are presented  on the table \ref{tab:utility-privacy}. When $p$ and $q$ are set with a smaller value, the system provides stronger privacy for use but achieves lower utility e.g., with $p = 0.3$ and $q = 0.3$,  $\epsilon = 1.7047$ and $\eta = 0.245$, whereas when $p$ and $q$ are set with a bigger value, the system provides higher utility but weaker privacy e.g., with $p = 0.9$ and $q = 0.9$,  $\epsilon = 3.1570$ and  $\eta = 0.0594$.
%
%
%\begin{table}[t!]
%\small
%\centering
%\begin{tabular}{c|c|c|c}
%\hline $p$ & $q$ & Accuracy loss ($\eta$) & Privacy Level ($\epsilon$) \\
%\hline
%\hline \multirow{3}{*}{0.3} & 0.3 & 0.2450 & 1.7047\\
%  & 0.6 & 0.2128 & 1.3862\\
%  & 0.9 & 0.1530 & 1.2527\\
%\hline \multirow{3}{*}{0.6} & 0.3 & 0.1154 & 2.5649\\
%  & 0.6 & 0.0986 & 2.0476\\
%  & 0.9 & 0.0902 & 1.7917\\
%\hline \multirow{3}{*}{0.9} & 0.3 & 0.0730 & 4.1820 \\
%  & 0.6 & 0.0682 & 3.5263\\
%  & 0.9 & 0.0594 & 3.1570\\
%\hline
%\end{tabular}
%\vspace{-2mm}
%\caption{The utility and the privacy guarantee of query results with different randomizing $p$ and $q$. The utility is measured by the query result's relative error (see expression~\ref{eq:accuracyloss}), and privacy is calculated by the level of achieved zero-knowledge privacy (see expression~\ref{eq:ezk}).  The number of original answers is set to $10,000$ with $80$\% of them are `yes'. The sampling parameter $r$ is set to $0.6$. Each result is generated after 100 independent runs.}
%\vspace{-2.5mm}
%\label{tab:utility-privacy}
%\end{table}
%
%\subsubsection{What is the effect of varying numbers of participated {\em Clients} on the utility?}
%Next, we analyze the impact of different numbers of participated {\em Clients} on the utility with constant sampling and randomizing parameters. For this experiment, we keep sampling and randomizing parameters--fixed. In detail, $p$, $q$ and $r$ are set to $0.9$ and the fraction of original answers are `yes' is fixed to $80$\%. Figure~\ref{fig:num-answers-error} depicts the effect of varying numbers of {\em Clients} on the utility. The result of this experiment shows that the processing answers of too few participated {\em Clients} could lead to very low utility (i.e., very high accuracy loss) of the query results.
%
%\subsubsection{What is the effect of varying fractions of origin truthful `yes' answers on the utility?}
%In the next experiment, we evaluate the impact of varying fractions of origin truthful `yes' answers on the utility. We measure the utility with different fractions of original truthful `yes' answers, meanwhile keep other parameters--sampling, randomizing parameters, and the total number of original answers--fixed. The number of original answers is set to $10,000$ and the sampling and randomizing parameters $p$, $q$ and $r$ are set to $0.9$. Figure~\ref{fig:num-answers-error} represents the experiment results. The system achieves higher utility as the fraction of original truthful `yes' answers increases. This is because of the randomized response mechanism. If the fraction of truthful answers being `yes' is high, then the utility of the query results generated based on randomized answers of {\em Clients} will be also high.
%
%\subsubsection{What is the encryption computation overhead compared to previous systems?}
%In privacy-preserving analytics systems, crypto operations are used to provide stronger privacy guarantees to users. However, the overhead of crypto operations is a major bottleneck of the system. Therefore, we conduct experiments to measure the computation overhead of \projecttitle and previous systems~\cite{RSA, Chen-2012, Paillier}. The crypto operations of previous system are RSA~\cite{RSA}, Goldwasser-Micali~\cite{Chen-2012}, and Paillier~\cite{Paillier}; whereas the crypto operations of \projecttitle is XOR operations.
%Note that, the Paillier-based approach~\cite{Paillier} is not resistant to the pollution attacks. Even a single malicious {\em Client} can substantially distort the query results in the Paillier-based system without any detection. Although the Paillier-based approach contains this weakness, we still want to add it in these experiments for the computation overhead comparison.
%
%We analyzed the computation overhead of crypto methods on various types of devices: 1) Android Galaxy mini III smartphone running Android 4.1.2 with a 1.5 GHz CPU, 2) MacBook Air laptop with a 2,2 GHz Intel Core i7 CPU, 8GB of RAM running OS X Yonsemite 10.10.2. 3) Linux server running Linux 3.15.0 with a 2.2 GHz CPU with 32 cores. In particular, we measured the number of cryto operations can be executed on each device per second. Table~\ref{tab:overhead} shows, not surprisingly, that the XOR operation of \projecttitle are extremely efficient compared to crypto methods of previous systems. In other words,  the XOR operations will not create any significant performance bottleneck in \projecttitle.
%
%
%\begin{table*}[t!]
%\small
%\centering
%\begin{tabular}{r|r|r|r|r|r|r}
%\hline
%                                                                           & \multicolumn{3}{c|}{Encryption}      & \multicolumn{3}{c}{Decryption}                \\ \hline 
%                                                                           & Phone    &  Laptop     & Server         & Phone          & Laptop          & Server \\ \hline \hline
%RSA in~\cite{RSA}           & 937      &   2,770       & 4,909         & 126            & 698              & 859              \\ \hline
%Goldwasser in~\cite{Chen-2012}   & 2,106    &  17,064    & 22,902        & 127            & 6,329           & 7,068           \\ \hline
%Paillier in~\cite{Paillier}     & 116       &  489         & 579             & 72              & 250              & 309              \\ \hline
%XOR in \projecttitle                                               & 15,026  &  943,902  & 1,351,937   & 3,262,186  & 16,519,076  & 22,678,285   \\ \hline
%\end{tabular}
%\vspace{-2mm}
%\caption{Computational overhead of cryptographic operations (\# operations / second).  The public-key crypto schemes use a 1024-bit key.}
%\vspace{-9mm}
%
%\label{tab:overhead}
%\end{table*}
%
%\subsubsection{What is the latency at {\em Proxies} compared to the previous system {\em SplitX}?}
%A previous system~\cite{Chen-2013}, namely {\em SplitX}, is also able to defeat the pollution attacks and contains similar components as \projecttitle. However, unlike \projecttitle, {\em SplitX} requires synchronization among system components to apply the randomized response mechanism to query answers at {\em Proxies} (in {\em SplitX}, the {\em Proxies} components are called {\em Mixes}). The synchronization creates a significant delay in processing query answers, and this prevents the usage of {\em SplitX} for stream analytics. We conducted experiments to measure the latency at {\em Mixes} of {\em SplitX} as well as {\em Proxies} of \projecttitle in processing query answers. Figure~\ref{fig:splitx-comparison} depicts the latency comparison in processing query answers at {\em Proxies} between {\em SplitX} and \projecttitle with different numbers of participated {\em Clients}. The log-log plot shows a not surprising result that the latency at {\em Mixes} of {\em Splitx} is significant higher than the latency at {\em Proxies} of \projecttitle. With $1,000,000$ {\em Clients}, the latency at {\em SplitX} is $40.276\ seconds$, while this value of \projecttitle is $6.209\ seconds$.
%  
%Figure~\ref{fig:case-splitx-comparison} depicts the latency comparison between {\em Mixes} (Splitx) and {\em Proxies} (PrivApprox).


==> figuresTex/fig-aggregator-throughput.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/throughput-aggregator.eps}
\caption{Aggregator throughput with the different numbers of nodes.}
%\vspace{-5mm}
\label{fig:aggregator-throughput}
\end{figure}


==> figuresTex/fig-benchmark-error.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.4\textwidth]{figuresTex/figures/error-benchmarks.eps}
\caption{The accuracy loss with different sampling and randomization parameters.  The number of answers is $10,000$ with 60\% of which being ``Yes'' answers.}
%\vspace{-5mm}
\label{fig:benchmark-error}
\end{figure}


==> figuresTex/fig-case-study-error.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/error-newyorktaxi.eps}
\caption{The accuracy loss with different numbers of sampling and randomizing parameters.}
%\vspace{-5mm}
\label{fig:case-study-error}
\end{figure}


==> figuresTex/fig-case-study-networktraffic.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/network-traffic.eps}
\caption{Total network traffic transferred to Proxies with different numbers of sampling fraction at Clients.}
%\vspace{-5mm}
\label{fig:network-traffic}
\end{figure}


==> figuresTex/fig-case-study-privacy.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/privacy-newyorktaxi.eps}
\caption{The privacy level with different numbers of sampling and randomizing parameters.}
%\vspace{-5mm}
\label{fig:case-study-privacy}
\end{figure}


==> figuresTex/fig-computation-model.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.35]{figuresTex/figures/computation-model}
\caption{Sliding window computation over data stream}
\label{fig:computation-model}
\end{figure}

==> figuresTex/fig-error-proof.tex <==
\begin{figure}
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/error-proof.eps}
\caption{The accuracy loss during the randomized response process and sampling process, separately; and the total accuracy loss after the two processes. The utility is measured by the query result's accuracy loss (see Equation~\ref{eq:accuracyloss}). The number of original answers is set to $10,000$ with $60\%$ of which being ``Yes'' answers. The accuracy loss of the randomized response process is measured separately by setting the sampling parameter to $100\%$ ($s = 1$) and the randomized response parameters $p$ and $q$ to $0.3$ and $0.6$, respectively, while the accuracy loss of the sampling process is measured without randomized response process by setting to $p$ to $1$. }
\vspace{-2mm}
\label{fig:error-proof}
\end{figure}

==> figuresTex/fig-fraction-yes-error.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/error-fraction-yes.eps}
\caption{The accuracy loss of query results with different fractions of original truthful ```Yes'' answers. The utility is measured by the query result's accuracy loss (see expression~\ref{eq:accuracyloss}).  The number of original answers is set to $10,000$. The sampling and randomizing parameters $r$, $p$, and $q$ are set to 0.9. Each result is generated after 100 independent runs.}
%\vspace{-5mm}
\label{fig:fraction-yes-error}
\end{figure}


==> figuresTex/fig-latency-sampling-aggregator.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/latency-sampling-aggregator.eps}
\caption{The latency of historical data processing with the different sampling fractions at Aggregator.}
%\vspace{-5mm}
\label{fig:latency-sampling-aggregator}
\end{figure}


==> figuresTex/fig-latency-sampling-fraction.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/latency-sampling-clients.eps}
\caption{Processing latency at Aggregator with the different sampling fractions at Clients.}
%\vspace{-5mm}
\label{fig:latency-sampling-franction}
\end{figure}


==> figuresTex/fig-negative-query.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.4\textwidth]{figuresTex/figures/negative-query.eps}
\caption{The accuracy loss of the native query and negative query results with different fractions of original truthful “Yes” answers. The utility is measured by the query result’s accuracy loss (see Equation 6). The number of original answers is set to $10,000$.}
%\vspace{-5mm}
\label{fig:negative-query}
\end{figure}


==> figuresTex/fig-num-answers-error.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/error-num-answers.eps}
\caption{The accuracy loss with different numbers of clients. The utility is measured by the query result's relative error (see expression~\ref{eq:accuracyloss}).  Before randomizing step, the fraction of original ``Yes'' answers is 80\% . the sampling and randomizing parameters $r$, $p$ and $q$ are set to $0.9$.  Each result is generated after 100 independent runs.}
%\vspace{-5mm}
\label{fig:num-answers-error}
\end{figure}


==> figuresTex/fig-otp-encryption.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.23,angle=-90]{figuresTex/figures/otp-encryption}
\caption{OTP-based encryption}
\label{fig:otp}
\end{figure}


==> figuresTex/fig-proxies-bitvector.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/throughput-proxies-bitvector.eps}
\caption{The throughput of proxies with different answer's bit-vector lengths.}
%\vspace{-5mm}
\label{fig:proxies-bitvector}
\end{figure}


==> figuresTex/fig-proxy-throughput.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/throughput-proxies.eps}
\caption{Proxy throughput with the different numbers of cores.}
%\vspace{-5mm}
\label{fig:proxy-throughput}
\end{figure}


==> figuresTex/fig-sampling-aggregator-error.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.45\textwidth]{figuresTex/figures/error-sampling-aggregator.eps}
\caption{The accuracy loss with different numbers of sampling fractions at aggregator}
%\vspace{-5mm}
\label{fig:case-study-error}
\end{figure}


==> figuresTex/fig-stratified-sampling.tex <==
\begin{figure}[t]
\centering
\includegraphics [width=0.4\textwidth]{figuresTex/figures/stratified-sampling.eps}
\caption{The average number of sampled data items of the three stream sources with different sampling fractions.}
%\vspace{-5mm}
\label{fig:stratified-sampling}
\end{figure}


==> figuresTex/fig-stratified-sampling1.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[scale=1.55]{figuresTex/figures/stratified.eps} 
  %\vspace{-4mm}
  \caption{The average number of sampled data items from three stream sources after stratified sampling with different sampling fractions.}
  \label{fig:stratified-sampling}
\end{figure}

==> figuresTex/fig-system-components.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.25]{figuresTex/figures/System-components}
\caption{\projecttitle system components}
\label{fig:sysComponents}
\end{figure}

